Proving LTL Properties of Bitvector Programs and Decompiled Binaries (Extended)

There is increasing interest in applying verification tools to programs that have bitvector operations (eg., binaries). SMT solvers, which serve as a foundation for these tools, have thus increased support for bitvector reasoning through bit-blasting and linear arithmetic approximations. In this paper we show that similar linear arithmetic approximation of bitvector operations can be done at the source level through transformations. Specifically, we introduce new paths that over-approximate bitvector operations with linear conditions/constraints, increasing branching but allowing us to better exploit the well-developed integer reasoning and interpolation of verification tools. We show that, for reachability of bitvector programs, increased branching incurs negligible overhead yet, when combined with integer interpolation optimizations, enables more programs to be verified. We further show this exploitation of integer interpolation in the common case also enables competitive termination verification of bitvector programs and leads to the first effective technique for LTL verification of bitvector programs. Finally, we provide an in-depth case study of decompiled ("lifted") binary programs, which emulate X86 execution through frequent use of bitvector operations. We present a new tool DarkSea, the first tool capable of verifying reachability, termination, and LTL of lifted binaries.

==> fig/fig_decp_syntax.tex <==
\begingroup
\input{fig/fig_decp_syntax_defs}
\lstMakeShortInline[style=boldinline]`
\[
\begin{array}{rcl}
	\pdec & \pdef & \stmt \por \labe `:` \stmt \por \goto ~ \labe; \\  

\end{array}
\]
\lstDeleteShortInline`
\endgroup


==> fig/fig_decp_syntax_expr.tex <==
\begingroup
\input{fig/fig_decp_syntax_defs}
\lstMakeShortInline[style=boldinline]`
\[
\begin{array}{rcl}
	\expr		    & \pdef & \lit \por \id \por (\expr) \por \const \por \func \por \nexpr \\ 
				    & \por & \bitexpr \por \binexpr \por \bitconst \\
                                    & \por & \ubitop \bitexpr \\
	\binexpr            & \pdef & \bitexpr ~\bitop~ \bitexpr \por \bitconst ~\bitop~ \bitexpr ~\por~ \expr ~\ariop~ \expr \\
	\bitexpr            & \pdef & \expr ~\logop~ \expr \por \idbit ~\bitop~ \bitexpr \por \bitexpr ~\bitop~ \bitexpr \\
                                    & \por & \idbit ~\bitop~ \idbit \por \bitexpr ~\bitop~ \idbit \\
	\ariop              & \pdef & `+` \por `-` \por `*` \por `/` \\
	\logop              & \pdef & `==` \por `!=` \por `<=` \por `<` \por `>` \por `>=` \\
	\bitop		    & \pdef & `&`  \por `^` \por `|` \\
	\ubitop		    & \pdef & `~`  \por `!` \\
	\bitconst	    & \pdef & `0`  \por `1` \\

\end{array}
\]
\lstDeleteShortInline`
\endgroup


==> fig/fig_ult_boogie_syntax_decl.tex <==
\begingroup
\input{fig/fig_ult_boogie_syntax_defs}
\lstMakeShortInline[style=boldinline]`
\[
\begin{array}{rcl}
	\prog			& \cfgdef & \decl^* \\
	\decl			& \cfgdef & \tdecl \cfgor \cdecl \cfgor \adecl \cfgor \fdecl \\ 
					& \cfgor  & \vdecl \cfgor \pdecl \cfgor \idecl \\
	
	\tdecl			& \cfgdef & `type`~\attr^*~`finite`^?~\id~\id^* `;` \\ 
					& \cfgor  & `type`~\attr^*~`finite`^?~\id~\id^*~`=`~\type `;`\\
	\type			& \cfgdef & `bool` \cfgor `int` \cfgor `real` \\
					& \cfgor  & `bv`[0-9]^+ \\
					& \cfgor  & `(`\type`)` \\
					& \cfgor  & \id~\type^? \\
					& \cfgor  & \typeargs^?~`[` \plus{\type} `]`~\type \\
					& \cfgor  & `{`~\plus{\varlist}~`}` \\
	\typeargs		& \cfgdef & `<` \plus{\id} `>` \\				
	
	\cdecl			& \cfgdef & `const`~\attr^*~`unique`^?~\plus{\id}~`:`~\type~\order^? `;`\\
	\adecl			& \cfgdef & `axiom`~\attr^*~\expr `;`\\
	
	\fdecl			& \cfgdef & `function`~\attr^*~\id~\fsig `;`\\
					& \cfgor  & `function`~\attr^*~\id~\fsig~`{`\expr~`}`\\
	\fsig			& \cfgdef & \typeargs^?~`() returns (` (\id~`:`)^?~\type `)` \\
					& \cfgor  & \typeargs^?~`(` \plus{\varlist} `) returns (` (\id~`:`)^?~\type `)` \\				
	
	
	\vdecl			& \cfgdef & `var`~\attr^*~\plus{\varlistwhere} `;`\\
	
	\varlist		& \cfgdef & \id~`:`~\type~(`,` \id~`:`~\type)^* \\
	\varlistwhere	& \cfgdef & \varlist~(`where`~\expr)^? \\
	
	\pdecl			& \cfgdef & `procedure`~\attr^*~\id~\psig`;`~\spec^*\\
					& \cfgor  & `procedure`~\attr^*~\id~\psig~\spec^*~\body\\
	\psig			& \cfgdef & \typeargs^?~`()`~\poutp^? \\
					& \cfgor  & \typeargs^?~`(`\plus{\varlistwhere}`)`~\poutp^? \\
	\poutp			& \cfgdef & `returns ()` \\
					& \cfgor  & `returns (`\plus{\varlistwhere}`)` \\

	\idecl			& \cfgdef & `implementation`~\attr^*~\id~\isig~\body\\
	\isig			& \cfgdef & \typeargs^?~`()`~\ioutp^? \\
					& \cfgor  & \typeargs^?~`(`\plus{\varlist}`)`~\ioutp^? \\
	\ioutp			& \cfgdef & `returns ()` \\
					& \cfgor  & `returns (`\plus{\varlist}`)` \\
						
	\body 			& \cfgdef & `{`\vdecl^*~\stmt^*~`};` \\
	
	\spec			& \cfgdef & `free`^?~`requires`~\expr`;`\\
					& \cfgor  & `free`^?~`ensures`~\expr`;`\\
					& \cfgor  & `free`^?~`modifies`~\plus{\id}`;`\\

	\order			& \cfgdef & `<:`~`complete`\\
					& \cfgdef & `<:`~`unique`^?~\plus{\id}~`complete`^?\\

	\attr			& \cfgdef & `{ :`~\id~`}` \cfgor `{ :`~\id~\plus{\attrarg}~`}` \\
	\attrarg		& \cfgdef & \expr \cfgor \str \\
	
\end{array}
\]
\lstDeleteShortInline`
\endgroup

==> fig/fig_ult_boogie_syntax_expr.tex <==
\begingroup
\input{fig/fig_ult_boogie_syntax_defs}
\lstMakeShortInline[style=boldinline]`
\[
\begin{array}{rcl}
	\expr		    & \cfgdef & \lit \cfgor \id \\ 
					& \cfgor  & \expr~\binop~\expr \cfgor \unop~\expr \cfgor `(`\expr`)` \\
				    & \cfgor  & `(if`~\expr~`then`~\expr~`else`~\expr`)` \\
				    & \cfgor  & `old(`\expr`)` \\
				    & \cfgor  & \id~`(`(\expr)^*`)` \\
				    & \cfgor  & \expr~`[`\plus{\expr} (`:=`~\expr)^?`]` \\
				    & \cfgor  & \expr~`[`\lit~`:`~\lit`]` \\
				    & \cfgor  & `(`\qop~\typeargs^?~\plus{\varlist}~`::`~\trigattr^*~\expr`)` \\
	\binop			& \cfgdef & `+` \cfgor `-` \cfgor `*` \cfgor `/` \cfgor `%` \\
				    & \cfgor  & `&&` \cfgor `||` \cfgor `==>` \cfgor `<==>` \\
				    & \cfgor  & `==` \cfgor `!=` \cfgor `<`   \cfgor `<=` \cfgor `>` \cfgor `>=` \\
				    & \cfgor  & `++`  \cfgor `<:` \\
	\unop		    & \cfgdef & `-`  \cfgor `!` \\
	\qop		    & \cfgdef & `forall`  \cfgor `exists` \\
	\lit			& \cfgdef & `true` \cfgor `false` \\
					& \cfgor  & `0` \cfgor `1` \cfgor `2` \cfgor \ldots \\
					& \cfgor  & `0.0` \cfgor `0.01`\ldots \cfgor `0.001`\ldots \cfgor \ldots \cfgor `1.0` \cfgor `1.01`\ldots \cfgor \ldots\\
					& \cfgor  & `0bv0` \cfgor `0bv1` \cfgor `1bv1` \cfgor `0bv2`\cfgor `1bv2` \cfgor `2bv2` \cfgor `3bv2` \cfgor \ldots\\
	\trigattr	    & \cfgdef & `{`~\plus{\expr}~`}` \cfgor \attr \\			
\end{array}
\]
\lstDeleteShortInline`
\endgroup

==> fig/fig_ult_boogie_syntax_stmt.tex <==
\begingroup
\input{fig/fig_ult_boogie_syntax_defs}
\lstMakeShortInline[style=boldinline]`
\[
\begin{array}{rcl}
	\stmt           & \cfgdef & `assume`~\expr `;` \\
				    & \cfgor  & `assert`~\expr`;` \\
				    & \cfgor  & `havoc`~\plus{\id}`;` \\
				    & \cfgor  & \plus{\lhs}~`:=`~\plus{\expr}`;`\\
				    & \cfgor  & `if (`\nexpr`){`~\stmt^*~`}`~\ifelse^?\\
				    & \cfgor  & `while (`\nexpr`)`~\loopinv^*~`{`\stmt^{*}~`}`\\
				    & \cfgor  & `break`~\id^?`;`\\
				    & \cfgor  & \id~`:`~\stmt^? \\
				    & \cfgor  & `goto`~\plus{\id}`;`\\
				    & \cfgor  & `call`~\clhs^?~\id~`();` \\
				    & \cfgor  & `call`~\clhs^?~\id~`(`\plus{\expr}`);` \\
				    & \cfgor  & `call`~`forall`~\id~`(`\nexpr^?`);` \\
				    & \cfgor  & `call`~`forall`~\id~`(`\plus{\expr}`);` \\
				    & \cfgor  & `return;`\\

	\lhs			& \cfgdef & \id \\
					& \cfgor  & \id`[` \plus{\expr} `]` \\
	\nexpr			& \cfgdef & `*` \cfgor \expr \\    
	\ifelse			& \cfgdef & `else {`~\stmt^*~`}` \\ 
					& \cfgor  & `else if (`\nexpr`){`~\stmt^*~`}`\ifelse^? \\
	\clhs			& \cfgdef & \plus{\id}~`:=` \\
	\loopinv		& \cfgdef & `free`^?~`invariant`~\expr`;` \\
	
\end{array}
\]
\lstDeleteShortInline`
\endgroup

==> tab/tab_eval_ltl_mcsema.tex <==
\begin{tabular}{lllcrcr}
    \toprule
    Benchmark                                       & Property & Expected & \multicolumn{2}{c}{\ultimate} & \multicolumn{2}{c}{\Tool}                   \\
                                                    &          &          & Time                          & Result                          & Time   & Result \\
    \cmidrule(lr){4-5}\cmidrule(lr){6-7}
    example3\_fail\_disable\_all.cbe.c              &          &          & 10.47s                        & \OK                             & 12.02s & \OK    \\
    example3\_succeed\_disable\_all.cbe.c           &          &          & 11.11s                        & \OK                             & 11.36s & \OK    \\
    PotentialMinimizeSEVPABug\_gccO0.mcsema.cbe.c   &          &          & 6.31s                         & \FAIL                           & 5.93s  & \FAIL  \\
    example2\_fail\_disable\_all.cbe.c              &          &          & 12.26s                        & \OK                             & 13.54s & \OK    \\
    someNonterminating\_gccO0.mcsema.cbe.c          &          &          & 4.57s                         & \FAIL                           & 4.92s  & \FAIL  \\
    01-exsec2\_true-valid-ltl.mcsema.false.c        &          &          & 6.31s                         & \FAIL                           & 5.79s  & \FAIL  \\
    acqrel.mcsema.false.c                           &          &          & 6.06s                         & \FAIL                           & 5.48s  & \FAIL  \\
    acqrel.mcsema.cbe.c                             &          &          & 5.17s                         & \FAIL                           & 5.38s  & \FAIL  \\
    example1\_fail\_disable\_all.cbe.c              &          &          & 13.06s                        & \OK                             & 13.44s & \OK    \\
    PotentialMinimizeSEVPABug\_gccO0.mcsema.false.c &          &          & 5.16s                         & \UNK                            & 5.25s  & \UNK   \\
    example1\_succeed\_disable\_all.cbe.c           &          &          & 11.22s                        & \OK                             & 11.11s & \OK    \\
    example2\_succeed\_disable\_all.cbe.c           &          &          & 14.24s                        & \OK                             & 14.15s & \OK    \\
    exsec2.mcsema.cbe.c                             &          &          & 4.92s                         & \FAIL                           & 4.96s  & \FAIL  \\
    exsec2.mcsema.false.c                           &          &          & 4.55s                         & \FAIL                           & 5.22s  & \FAIL  \\
    01-exsec2\_true-valid-ltl.mcsema.cbe.c          &          &          & 4.45s                         & \FAIL                           & 4.56s  & \FAIL  \\
    simple3\_gccO0.mcsema.false.c                   &          &          & 4.96s                         & \FAIL                           & 4.87s  & \FAIL  \\
    simple3\_gccO0.mcsema.cbe.c                     &          &          & 4.97s                         & \FAIL                           & 5.82s  & \FAIL  \\
\end{tabular}

==> tab/tab_eval_ltl_simplify.tex <==
\begin{tabular}{lllcrcr}
    \toprule
    Benchmark                                           & Property & Expected & \multicolumn{2}{c}{\ultimate} & \multicolumn{2}{c}{\Tool}                    \\
                                                        &          &          & Time                          & Result                          & Time    & Result \\
    \cmidrule(lr){4-5}\cmidrule(lr){6-7}
    01-exsec2\_true-valid-ltl.sliced.cbe.c.instr.c      &          &          & 9.62s                         & \OK                             & 8.39s   & \OK    \\
    someNonterminating\_gccO0.sliced.int.c              &          &          & 11.54s                        & \UNK                            & 10.03s  & \NOK   \\
    example2\_succeed\_enable\_all.sliced.cbe.c.instr.c &          &          & 12.40s                        & \UNK                            & 9.61s   & \OK    \\
    acqrel.simplify.sliced.false.c.instr.c              &          &          & 50.95s                        & \UNK                            & 900.55s & \TOUT  \\
    PotentialMinimizeSEVPABug\_gccO0.sliced.false.c     &          &          & 12.49s                        & \UNK                            & 51.38s  & \NOK   \\
    example3\_succeed\_enable\_all.sliced.cbe.c.instr.c &          &          & 6.32s                         & \UNK                            & 5.52s   & \OK    \\
    PotentialMinimizeSEVPABug\_gccO0.sliced.int.c       &          &          & 10.24s                        & \UNK                            & 26.56s  & \OK    \\
    example1\_fail\_enable\_all.sliced.cbe.c.instr.c    &          &          & 7.04s                         & \NOK                            & 5.97s   & \NOK   \\
    example1\_succeed\_enable\_all.sliced.cbe.c.instr.c &          &          & 8.58s                         & \OK                             & 9.01s   & \OK    \\
    exsec2.simplify.sliced.cbe.c.instr.c                &          &          & 5.42s                         & \OK                             & 5.11s   & \OK    \\
    01-exsec2\_true-valid-ltl.sliced.false.c.instr.c    &          &          & 8.58s                         & \UNK                            & 10.93s  & \NOK   \\
    exsec2.simplify.sliced.false.c.instr.c              &          &          & 5.82s                         & \NOK                            & 8.09s   & \NOK   \\
    example3\_fail\_enable\_all.sliced.cbe.c.instr.c    &          &          & 7.42s                         & \UNK                            & 6.43s   & \NOK   \\
    acqrel.simplify.sliced.cbe.c.instr.c                &          &          & 10.03s                        & \OK                             & 10.10s  & \OK    \\
    simple3\_gccO0.sliced.false.c                       &          &          & 58.29s                        & \UNK                            & 380.22s & \NOK   \\
    simple3\_gccO0.sliced.int.c                         &          &          & 53.49s                        & \UNK                            & 18.91s  & \OK    \\
    example2\_fail\_enable\_all.sliced.cbe.c.instr.c    &          &          & 12.49s                        & \UNK                            & 12.45s  & \NOK   \\
\end{tabular}

==> tab/tab_eval_old_ltl_bithacks.tex <==
\begin{tabular}{lllcrcr}
    \toprule
                                            &                              &          & \multicolumn{2}{c}{\sautomizer} & \multicolumn{2}{c}{\Tool}                    \\
                                            & Property                     & Expected & Time                            & Result                          & Time    & Result \\
    \cmidrule(r){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(l){7-7}
    consecutive-zero-bits-trailing\_false.c & $\lozenge y = 1$             & \NOK     & 11.67s                          & \UNK                            & 16.24s  & \UNK   \\
    counting-bits-BK\_false.c               & $\square(\lozenge y \leq 1)$ & \NOK     & 13.62s                          & \UNK                            & 15.75s  & \NOK   \\
    counting-bits-BK1\_false.c              & $\square(\lozenge y \geq 0)$ & \NOK     & 12.66s                          & \UNK                            & 15.97s  & \NOK   \\
    counting-bits-set\_false.c              & $\lozenge y \geq 1$          & \NOK     & 16.25s                          & \UNK                            & 15.54s  & \NOK   \\
    display-bit\_false.c                    & $\lozenge y < 0$             & \NOK     & 40.80s                          & \UNK                            & 89.33s  & \NOK   \\
    display-bit1\_false.c                   & $\lozenge y > 1$             & \NOK     & 34.03s                          & \UNK                            & 86.49s  & \NOK   \\
    parity\_false.c                         & $\lozenge y \geq 1$          & \NOK     & 32.67s                          & \UNK                            & 14.47s  & \NOK   \\
    reverse-bits1\_false.c                  & $\lozenge n < 0$             & \NOK     & 10.95s                          & \UNK                            & 13.74s  & \NOK   \\
    consecutive-zero-bits-trailing.c        & $\lozenge y \geq 1$          & \OK      & 12.50s                          & \UNK                            & 13.18s  & \OK    \\
    counting-bits-BK.c                      & $\square(\lozenge y \leq 1)$ & \OK      & 13.39s                          & \UNK                            & 15.85s  & \OK    \\
    counting-bits-BK1.c                     & $\square(\lozenge y \geq 0)$ & \OK      & 12.70s                          & \UNK                            & 13.83s  & \OK    \\
    counting-bits-set.c                     & $\lozenge y \geq 1$          & \OK      & 16.06s                          & \UNK                            & 16.56s  & \OK    \\
    display-bit.c                           & $\lozenge y \geq 32$         & \OK      & 39.88s                          & \UNK                            & 19.35s  & \OK    \\
    display-bit1.c                          & $\lozenge y \geq 1$          & \OK      & 33.94s                          & \UNK                            & 14.46s  & \OK    \\
    parity.c                                & $\lozenge y \geq 1$          & \OK      & 32.73s                          & \UNK                            & 13.20s  & \OK    \\
    reverse-bits1.c                         & $\lozenge n < 0$             & \OK      & 11.80s                          & \UNK                            & 12.97s  & \UNK   \\
    %% not helping, but keep them or manually remove them from overview table
    consecutive-zero-bits.c                 & $\lozenge y \geq 1$          & \OK      & 9.45s                           & \OK                             & 11.05s  & \OK    \\
    counting-bits-lookup.c                  & $\lozenge y \geq 1$          & \OK      & 900.42s                         & \TOUT                           & 900.42s & \TOUT  \\
    interleave-bits.c                       & $\lozenge y \geq 1$          & \OK      & 22.62s                          & \UNK                            & 428.39s & \UNK   \\
    logbase2-N-bit1.c                       & $\lozenge y \geq 1$          & \OK      & 24.89s                          & \UNK                            & 902.19s & \TOUT  \\
    logbase2.c                              & $\lozenge y \geq 1$          & \OK      & 13.71s                          & \UNK                            & 14.33s  & \UNK   \\
    modulus-division.c                      & $\lozenge y > 1$             & \OK      & 13.12s                          & \UNK                            & 11.79s  & \UNK   \\
    reverse-N-bit.c                         & $\lozenge y \geq 1$          & \OK      & 12.38s                          & \OK                             & 51.61s  & \OK    \\
    reverse-bits.c                          & $\lozenge n \geq 1$          & \OK      & 13.37s                          & \UNK                            & 13.36s  & \UNK   \\
    \bottomrule
\end{tabular}


==> tab/tab_eval_old_ltl_other.tex <==
\begin{tabular}{lllcccc}
    \toprule
                         &                           &          & \multicolumn{2}{c}{\sautomizer} & \multicolumn{2}{c}{\Tool}                   \\
                         & Property                  & Expected & Time                            & Result                          & Time   & Result \\
    \cmidrule(r){2-2}\cmidrule(lr){3-3}    \cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(l){7-7}
    xor\_guard.c         & $\lozenge n < 0$          & \OK      & 12.61s                          & \UNK                            & 11.07s & \OK    \\
    xor\_stem1.c         & $\lozenge n < 0$          & \OK      & 11.24s                          & \UNK                            & 9.83s  & \OK    \\
    or\_stem.c           & $\lozenge n < 0$          & \OK      & 10.80s                          & \UNK                            & 10.42s & \OK    \\
    and\_stem2.c         & $\lozenge n > 0$          & \OK      & 11.01s                          & \UNK                            & 11.39s & \OK    \\
    xor\_loop.c          & $\lozenge n < 0$          & \OK      & 11.38s                          & \UNK                            & 15.71s & \OK    \\
    com\_loop.c          & $\lozenge y < 0$          & \OK      & 10.78s                          & \UNK                            & 10.33s & \OK    \\
    and\_guard1.c        & $\lozenge n > 0$          & \OK      & 13.90s                          & \UNK                            & 10.69s & \OK    \\
    com\_stem.c          & $\square(\lozenge y=1)$   & \OK      & 11.39s                          & \UNK                            & 11.04s & \OK    \\
    and\_loop1.c         & $\lozenge z < 0$          & \OK      & 14.17s                          & \UNK                            & 11.29s & \OK    \\
    and\_guard.c         & $\lozenge n < 0$          & \OK      & 11.19s                          & \UNK                            & 10.76s & \UNK   \\
    and\_stem1.c         & $\lozenge n < 0$          & \OK      & 10.11s                          & \UNK                            & 9.96s  & \OK    \\
    xor\_stem.c          & $\lozenge n < 0$          & \OK      & 10.32s                          & \UNK                            & 9.61s  & \OK    \\
    or\_loop.c           & $\square(\lozenge n < 0)$ & \OK      & 11.06s                          & \UNK                            & 14.90s & \OK    \\
    and\_guard2.c        & $\lozenge z \geq 100 $    & \OK      & 13.82s                          & \UNK                            & 14.74s & \OK    \\
    and\_loop.c          & $\lozenge y \geq 1$       & \OK      & 10.80s                          & \UNK                            & 11.57s & \OK    \\
    or\_loop1.c          & $\square(\lozenge n < 0)$ & \OK      & 13.05s                          & \UNK                            & 12.07s & \OK    \\
    or\_guard.c          & $\lozenge n < 0$          & \OK      & 9.71s                           & \UNK                            & 9.59s  & \OK    \\
    and\_stem.c          & $\lozenge n < 0$          & \OK      & 10.46s                          & \UNK                            & 11.37s & \UNK   \\
    and\_guard4.c        & $\lozenge n > 0$          & \OK      & 15.08s                          & \UNK                            & 10.46s & \OK    \\
    or\_loop2.c          & $\lozenge n < 0$          & \OK      & 12.44s                          & \UNK                            & 10.89s & \OK    \\
    or\_guard\_false.c   & $\lozenge n < 0$          & \NOK     & 10.68s                          & \UNK                            & 10.95s & \NOK   \\
    and\_guard4\_false.c & $\lozenge n > 0$          & \NOK     & 14.15s                          & \UNK                            & 11.11s & \NOK   \\
    com\_loop\_false.c   & $\lozenge y < 0$          & \NOK     & 10.60s                          & \UNK                            & 10.80s & \NOK   \\
    xor\_stem1\_false.c  & $\lozenge n < 0$          & \NOK     & 10.67s                          & \UNK                            & 11.19s & \NOK   \\
    and\_guard\_false.c  & $\lozenge y > 0$          & \NOK     & 10.19s                          & \UNK                            & 11.19s & \NOK   \\
    xor\_guard\_false.c  & $\lozenge n > 0$          & \NOK     & 11.29s                          & \UNK                            & 10.85s & \NOK   \\
    com\_stem\_false.c   & $\square(\lozenge y < 0)$ & \NOK     & 17.42s                          & \UNK                            & 17.46s & \NOK   \\
    or\_loop2\_false.c   & $\lozenge n > 0$          & \NOK     & 11.98s                          & \UNK                            & 13.15s & \NOK   \\
    and\_guard1\_false.c & $\lozenge n > 0$          & \NOK     & 7.51s                           & \UNK                            & 7.85s  & \UNK   \\
    and\_stem1\_false.c  & $\lozenge n < 0$          & \NOK     & 10.73s                          & \UNK                            & 11.90s & \NOK   \\
    and\_stem\_false.c   & $\lozenge n < 0$          & \NOK     & 11.17s                          & \UNK                            & 11.15s & \NOK   \\
    xor\_stem\_false.c   & $\lozenge n < 0$          & \NOK     & 10.92s                          & \UNK                            & 10.60s & \NOK   \\
    or\_loop\_false.c    & $\square(\lozenge n < 0)$ & \NOK     & 11.40s                          & \UNK                            & 14.88s & \NOK   \\
    or\_loop1\_false.c   & $\square(\lozenge n < 0)$ & \NOK     & 13.41s                          & \UNK                            & 12.71s & \NOK   \\
    and\_guard2\_false.c & $\lozenge z \geq 100$     & \NOK     & 13.98s                          & \UNK                            & 10.19s & \NOK   \\
    and\_loop\_false.c   & $\lozenge y \geq 1$       & \NOK     & 11.10s                          & \UNK                            & 12.25s & \NOK   \\
    xor\_loop\_false.c   & $\lozenge n < 0$          & \NOK     & 10.60s                          & \UNK                            & 14.34s & \NOK   \\
    and\_stem2\_false.c  & $\lozenge n > 0$          & \NOK     & 11.19s                          & \UNK                            & 12.03s & \NOK   \\
    or\_stem\_false.c    & $\lozenge n < 0$          & \NOK     & 11.14s                          & \UNK                            & 13.03s & \NOK   \\
    and\_loop1\_false.c  & $\lozenge z < 0$          & \NOK     & 14.55s                          & \UNK                            & 14.34s & \NOK   \\
    \bottomrule
\end{tabular}

==> tab/tab_eval_reach_smt.tex <==

%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
%% \begin{table}[!htp]\centering
%%   \caption{SMT Solver Performance}
%%   \label{tab: reach}
%% \scriptsize
\begin{tabular}{lrrrrrrrrrrrrrrrrrr}
  \toprule
  &\multicolumn{2}{c}{\textbf{BV WOLF MathSAT}} &\multicolumn{2}{c}{\textbf{BV WOLF Z3}} &\multicolumn{2}{c}{\textbf{BV WOLF CVC4}} &\multicolumn{3}{c}{\textbf{DarkSea MathSAT}} &\multicolumn{3}{c}{\textbf{DarkSea Z3}} &\multicolumn{3}{c}{\textbf{DarkSea CVC4}} &\multicolumn{2}{c}{\textbf{DarkSea SmtInterpol}} \\ \cmidrule{2-18}
  Benchmark &Time &Res &Time &Res &Time &Res &single/without SmtInterpolCraig &Time &Res &Single &Time &Res &Single &Time &Res &Time &Res \\\cmidrule{1-18}
logic\_and.c &\cellcolor[HTML]{A8A8A8}537.74 &\textbf{true} &624.51 &true &639.92 &true &\cellcolor[HTML]{A8A8A8}13225.74 &\cellcolor[HTML]{A8A8A8}353.04 &true &677.15 &\cellcolor[HTML]{A8A8A8}78.37 &true &13462.73 &\cellcolor[HTML]{A8A8A8}403.54 &true &\cellcolor[HTML]{A8A8A8}75.14 &true \\\cmidrule{1-18}
logic\_and\_false.c &\cellcolor[HTML]{A8A8A8}409.01 &\cellcolor[HTML]{A8A8A8}false &406.63 &false &435.67 &false &\cellcolor[HTML]{A8A8A8}280.58 &\cellcolor[HTML]{A8A8A8}65.67 &false &271.24 &\cellcolor[HTML]{A8A8A8}37.38 &false &287.13 &\cellcolor[HTML]{A8A8A8}54.26 &false &\cellcolor[HTML]{A8A8A8}15.34 &false \\\cmidrule{1-18}
logic\_or.c &\cellcolor[HTML]{A8A8A8}712.1 &\textbf{true} &720.84 &true &618.93 &true &\cellcolor[HTML]{A8A8A8}582.79 &\cellcolor[HTML]{A8A8A8}72.13 &true &403.36 &\cellcolor[HTML]{A8A8A8}62.56 &true &585.91 &\cellcolor[HTML]{A8A8A8}99.35 &true &\cellcolor[HTML]{A8A8A8}66.72 &true \\\cmidrule{1-18}
logic\_or\_false.c &\cellcolor[HTML]{A8A8A8}434.95 &\cellcolor[HTML]{A8A8A8}false &422.25 &false &419.65 &false &\cellcolor[HTML]{A8A8A8}235.23 &\cellcolor[HTML]{A8A8A8}19.67 &false &240.66 &\cellcolor[HTML]{A8A8A8}11.21 &false &258.91 &\cellcolor[HTML]{A8A8A8}22.01 &false &\cellcolor[HTML]{A8A8A8}9.91 &false \\\cmidrule{1-18}
logic\_xor.c &\cellcolor[HTML]{A8A8A8}598.66 &\textbf{true} &568.22 &true &780.76 &true &\cellcolor[HTML]{A8A8A8}660.49 &\cellcolor[HTML]{A8A8A8}1134.92 &true &450.08 &\cellcolor[HTML]{A8A8A8}110.32 &true &596.71 &\cellcolor[HTML]{A8A8A8}128.26 &true &\cellcolor[HTML]{A8A8A8}107.89 &true \\\cmidrule{1-18}
logic\_xor\_false.c &\cellcolor[HTML]{A8A8A8}414.4 &\cellcolor[HTML]{A8A8A8}false &426.02 &false &407.5 &false &\cellcolor[HTML]{A8A8A8}230.79 &\cellcolor[HTML]{A8A8A8}16.3 &false &253.14 &\cellcolor[HTML]{A8A8A8}18.51 &false &265.95 &\cellcolor[HTML]{A8A8A8}21.66 &false &\cellcolor[HTML]{A8A8A8}10.91 &false \\\cmidrule{1-18}
logic\_cmpl.c &\cellcolor[HTML]{A8A8A8}585.28 &\cellcolor[HTML]{A8A8A8}true &512.98 &true &488.52 &true &\cellcolor[HTML]{A8A8A8}363.17 &\cellcolor[HTML]{A8A8A8}55.41 &true &347.08 &\cellcolor[HTML]{A8A8A8}60.97 &true &420.33 &\cellcolor[HTML]{A8A8A8}58.97 &true &\cellcolor[HTML]{A8A8A8}60.42 &true \\\cmidrule{1-18}
logic\_cmpl\_false.c &\cellcolor[HTML]{A8A8A8}417.52 &\cellcolor[HTML]{A8A8A8}false &406.49 &false &455.91 &false &\cellcolor[HTML]{A8A8A8}226.75 &\cellcolor[HTML]{A8A8A8}16.99 &false &255.24 &\cellcolor[HTML]{A8A8A8}11.67 &false &252.85 &\cellcolor[HTML]{A8A8A8}11.88 &false &\cellcolor[HTML]{A8A8A8}10.61 &false \\\cmidrule{1-18}
and\_loop.c &\cellcolor[HTML]{A8A8A8}638.41 &\cellcolor[HTML]{A8A8A8}true &611.75 &true &674.17 &true &\cellcolor[HTML]{A8A8A8}419.54 &\cellcolor[HTML]{A8A8A8}58.5 &true &425.21 &\cellcolor[HTML]{A8A8A8}57.27 &true &418.08 &\cellcolor[HTML]{A8A8A8}67.13 &true &\cellcolor[HTML]{A8A8A8}77.34 &true \\\cmidrule{1-18}
and\_loop\_false.c &\cellcolor[HTML]{A8A8A8}378.45 &\cellcolor[HTML]{A8A8A8}false &440.33 &false &418.11 &false &\cellcolor[HTML]{A8A8A8}265.27 &\cellcolor[HTML]{A8A8A8}17.44 &false &244.95 &\cellcolor[HTML]{A8A8A8}16.21 &false &254.27 &\cellcolor[HTML]{A8A8A8}16.17 &false &\cellcolor[HTML]{A8A8A8}10.83 &false \\\cmidrule{1-18}

{\textbf{BitHacks reach?}} & & & & & & & & & & & & & & & & & \\
parity.c &1842.22 &true &1774.06 &true &1846.72 &true &1016.47 &\cellcolor[HTML]{A8A8A8}286.23 &true &1059.09 &\cellcolor[HTML]{A8A8A8}257.23 &true &1057.34 &\cellcolor[HTML]{A8A8A8}283.44 &true &\cellcolor[HTML]{A8A8A8}235.36 &true \\\cmidrule{1-18}
consecutive-zero-bits-trailing.c &581.64 &true &565.43 &true &603.69 &true &571.31 &\cellcolor[HTML]{A8A8A8}287.68 &true &496.78 &\cellcolor[HTML]{A8A8A8}251.83 &true &563.79 &\cellcolor[HTML]{A8A8A8}292.41 &true &\cellcolor[HTML]{A8A8A8}300.34 &true \\\cmidrule{1-18}
counting-bits-BK.c &526.81 &true &502.33 &true &500.36 &true &504.37 &\cellcolor[HTML]{A8A8A8}103.16 &true &520.15 &\cellcolor[HTML]{A8A8A8}132.48 &true &498.12 &\cellcolor[HTML]{A8A8A8}142.33 &true &\cellcolor[HTML]{A8A8A8}133.66 &true \\\cmidrule{1-18}
counting-bits-BK1.c &-- &ERROR &-- &ERROR &-- &ERROR &1148.53 &\cellcolor[HTML]{A8A8A8}312.29 &true &1182.49 &\cellcolor[HTML]{A8A8A8}295.17 &true &1186.16 &\cellcolor[HTML]{A8A8A8}265.61 &true &\cellcolor[HTML]{A8A8A8}265.5 &true \\\cmidrule{1-18}
counting-bits-set.c &-- &ERROR &-- &ERROR &-- &ERROR &1665.15 &\cellcolor[HTML]{A8A8A8}704.62 &true &1635.99 &\cellcolor[HTML]{A8A8A8}683.97 &true &1570.21 &\cellcolor[HTML]{A8A8A8}572.95 &true &\cellcolor[HTML]{A8A8A8}637.88 &true \\\cmidrule{1-18}
display-bit.c &-- &ERROR &-- &ERROR &-- &ERROR &539.11 &\cellcolor[HTML]{A8A8A8}112.27 &true &500.82 &\cellcolor[HTML]{A8A8A8}131.52 &true &640.71 &\cellcolor[HTML]{A8A8A8}99.56 &true &\cellcolor[HTML]{A8A8A8}87.18 &true \\\cmidrule{1-18}
display-bit1.c &-- &ERROR &-- &ERROR &-- &ERROR &1982.92 &\cellcolor[HTML]{A8A8A8}1012.65 &true &1912.14 &\cellcolor[HTML]{A8A8A8}617.57 &true &1656.48 &\cellcolor[HTML]{A8A8A8}665.14 &true &\cellcolor[HTML]{A8A8A8}402.54 &true \\\cmidrule{1-18}
reverse-bits1.c &931.6 &true &923.87 &true &1048.93 &true &1647.29 &\cellcolor[HTML]{A8A8A8}308.15 &true &1505.7 &\cellcolor[HTML]{A8A8A8}452.09 &true &1570.04 &\cellcolor[HTML]{A8A8A8}373.03 &true &\cellcolor[HTML]{A8A8A8}377.9 &true \\\cmidrule{1-18}
& & & & & & & &\cellcolor[HTML]{A8A8A8} & & &\cellcolor[HTML]{A8A8A8} & & &\cellcolor[HTML]{A8A8A8} & &\cellcolor[HTML]{A8A8A8} & \\
parity\_false.c &-- &ERROR &-- &ERROR &-- &ERROR &1141.72 &\cellcolor[HTML]{A8A8A8}209.24 &false &1331.95 &\cellcolor[HTML]{A8A8A8}245.76 &false &1356.4 &\cellcolor[HTML]{A8A8A8}229.52 &false &\cellcolor[HTML]{A8A8A8}103.49 &false \\\cmidrule{1-18}
consecutive-zero-bits-trailing\_false.c &366.86 &false &397.5 &false &430.79 &false &400.38 &\cellcolor[HTML]{A8A8A8}25.77 &false &397.67 &\cellcolor[HTML]{A8A8A8}23.11 &false &396.06 &\cellcolor[HTML]{A8A8A8}20.72 &false &\cellcolor[HTML]{A8A8A8}14.12 &false \\\cmidrule{1-18}
counting-bits-BK\_false.c &-- &ERROR &-- &ERROR &-- &ERROR &1261.87 &\cellcolor[HTML]{A8A8A8}314.57 &false &1347.02 &\cellcolor[HTML]{A8A8A8}263.21 &false &1441.33 &\cellcolor[HTML]{A8A8A8}219.64 &false &\cellcolor[HTML]{A8A8A8}141.97 &false \\\cmidrule{1-18}
counting-bits-BK1\_false.c &-- &ERROR &-- &ERROR &-- &ERROR &367.24 &\cellcolor[HTML]{A8A8A8}27.88 &false &385.18 &\cellcolor[HTML]{A8A8A8}17.34 &false &407.49 &\cellcolor[HTML]{A8A8A8}33.82 &false &\cellcolor[HTML]{A8A8A8}17.13 &false \\\cmidrule{1-18}
counting-bits-set\_false.c &-- &ERROR &-- &ERROR &-- &ERROR &1305.01 &\cellcolor[HTML]{A8A8A8}315.49 &false &1295.98 &\cellcolor[HTML]{A8A8A8}205.7 &false &1415.43 &\cellcolor[HTML]{A8A8A8}248.51 &false &\cellcolor[HTML]{A8A8A8}153.92 &false \\\cmidrule{1-18}
display-bit\_false.c &-- &ERROR &-- &ERROR &-- &ERROR &13607.19 &\cellcolor[HTML]{A8A8A8}34931.2 &false &13877.29 &\cellcolor[HTML]{A8A8A8}58371.82 &false &13692.86 &\cellcolor[HTML]{A8A8A8}28152.31 &false &\cellcolor[HTML]{A8A8A8}36291.41 &false \\\cmidrule{1-18}
display-bit1\_false.c &-- &ERROR &-- &ERROR &-- &ERROR &13954.05 &\cellcolor[HTML]{A8A8A8}21377.58 &false &13955.51 &\cellcolor[HTML]{A8A8A8}31958.83 &false &14038.53 &\cellcolor[HTML]{A8A8A8}56958.17 &false &\cellcolor[HTML]{A8A8A8}44254.38 &false \\\cmidrule{1-18}
reverse-bits1\_false.c &-- &ERROR &-- &ERROR &-- &ERROR &1029.91 &\cellcolor[HTML]{A8A8A8}69.35 &false &929.5 &\cellcolor[HTML]{A8A8A8}83.05 &false &866.34 &\cellcolor[HTML]{A8A8A8}59.89 &false &\cellcolor[HTML]{A8A8A8}154.5 &false \\\midrule
\bottomrule
\end{tabular}
%% \end{table}


==> tab/tab_eval_reach_smt2.tex <==
\begin{tabular}{|l|r|rr|r|rr|r|rr|}
\hline
& \mathsat & \multicolumn{2}{c|}{\mathsat+BwB} & Z3 & \multicolumn{2}{c|}{Z3+BwB} & CVC4 & \multicolumn{2}{c|}{CVC4+BwB} \\
{\bf Benchmark} &  & No Itp & Itp &  & No Itp & Itp &  & No Itp & Itp \\
\hline
\hline
logic\_and.c & 617 & 1967 & 399 & 615 & 1905 & 344 & 686 & 2164 & 360 \\
logic\_and\_false.c & 401 & 423 & 216 & 389 & 405 & 213 & 438 & 426 & 207 \\
logic\_or.c & 645 & 776 & 328 & 653 & 730 & 358 & 676 & 769 & 362 \\
logic\_or\_false.c & 391 & 891 & 416 & 412 & 913 & 371 & 428 & 860 & 443 \\
logic\_xor.c & 612 & 891 & 416 & 624 & 913 & 371 & 633 & 860 & 443 \\
logic\_xor\_false.c & 386 & 396 & 262 & 422 & 394 & 223 & 398 & 425 & 217 \\
logic\_cmpl.c & 542 & 702 & 356 & 498 & 716 & 425 & 649 & 657 & 377 \\
logic\_cmpl\_false.c & 367 & 375 & 213 & 397 & 387 & 245 & 441 & 420 & 210 \\
and\_loop.c & 679 & 857 & 357 & 701 & 884 & 372 & 742 & 859 & 314 \\
and\_loop\_false.c & 389 & 793 & 396 & 435 & 839 & 339 & 462 & 998 & 326 \\
and\_reach1.c & 740 & 962 & 387 & 758 & 909 & 358 & 717 & 976 & 338 \\
parity.c & 2092 & 1108 & 449 & 2177 & 1136 & 471 & 2127 & 1138 & 508 \\
consec-zr-bits-trail.c & 616 & 660 & 380 & 630 & 661 & 424 & 695 & 715 & 440 \\
counting-bits-BK.c & 646 & 682 & 288 & 570 & 698 & 360 & 672 & 665 & 365 \\
counting-bits-BK1.c & 1259 & 19735 & 478 & 1090 & 19362 & 460 & 1123 & 2382 & 526 \\
counting-bits-set.c & 1257 & 1602 & 853 & 1196 & 1607 & 834 & 1090 & 1650 & 872 \\
reverse-bits1.c & 1190 & 1814 & 551 & 1225 & 1923 & 615 & 1220 & 1789 & 608 \\
parity\_false.c & 893 & 1152 & 417 & 917 & 1154 & 407 & 897 & 1176 & 371 \\
consec-zr-bits-trail\_false.c & 350 & 389 & 178 & 415 & 376 & 193 & 374 & 377 & 202 \\
counting-bits-BK\_false.c & 1054 & 1127 & 394 & 1183 & 1134 & 401 & 1196 & 1294 & 400 \\
counting-bits-BK1\_false.c & 364 & 360 & 196 & 394 & 423 & 173 & 431 & 475 & 213 \\
counting-bits-set\_false.c & 1226 & 1120 & 457 & 1133 & 1184 & 454 & 1266 & 1361 & 426 \\
reverse-bits1\_false.c & 403 & 868 & 425 & 395 & 977 & 431 & 495 & 966 & 369 \\
\hline
\hline
{\bf Total Time} & 17,118 & 39,651 & 8,812 & 17,229 & 39,630 & 8,844 & 17,855 & 23,400 & 8,898 \\
\hline
{\bf Slowdown/Speedup}: & & 0.4 & {\bf 4.5} & & 0.4 & {\bf 4.5} & & 0.8 & {\bf 2.6} \\
\hline
\end{tabular}


==> tab/tab_eval_reach_smt_bitvectors.tex <==
\begin{tabular}{lr@{\hspace{1em}}r@{\hspace{1em}}r@{\hspace{1em}}r@{\hspace{1em}}r@{\hspace{1em}}r@{\hspace{1em}}c}
    \toprule
    & \multicolumn{4}{c}{Integer} & \multicolumn{3}{c}{Bitvector}                                                             \\
    \cmidrule(r){2-5}\cmidrule{6-8}
             & \rheader{\bwb SItp+\zzz}
             & \rheader{SItp+\zzz}
             & \rheader{\bwb MS Itp}
             & \rheader{\bwb MS}
             & \rheader{MS Itp}
             & \rheader{MS}
             & \rheader{MS, \cvc, \zzz}                                                                                                \\

             \cmidrule(r){2-2}
             \cmidrule(r){3-3}
             \cmidrule(r){4-4}
             \cmidrule(r){5-5}
             \cmidrule(r){6-6}
             \cmidrule(r){7-7}
             \cmidrule{8-8}

    \OK      & 15 & 47 & 46 & 46 & 53        & 54         & 53         \\
    \NOK     & 5 & 23 & 23 & 24 & 30        & 39         & 38         \\
    \UNK     & 32 & 35 & 11 & 32 & -         & 6          & 5          \\
    \TOUT    & 13 & 30 & 4  & 40 & 13        & 35         & 38         \\
    \OOM     & 1  & 4  & 2  & 2  & 2         & 1          & 1          \\
    \FAIL    & 8  & 5  & 58 & -  & 46        & 9          & 9          \\
    
    % \midrule
    %   & 14,510.35s & 14,457.25s & 5,016.94s & 16,470.74s & 8,246.31s & 15,806.49s & 15,689.53s \\
    \midrule
    \OK,\NOK & 20 & 70 & 69 & 70 & 83 & 93 &  91 \\
    \bottomrule
\end{tabular}



==> tab/tab_eval_reach_smt_controlflow.tex <==
\begin{tabular}{lr@{\hspace{1em}}r@{\hspace{1em}}r@{\hspace{1em}}r@{\hspace{1em}}r@{\hspace{1em}}r@{\hspace{1em}}c}
    \toprule
    & \multicolumn{4}{c}{Integer} & \multicolumn{3}{c}{Bitvector}                                                             \\
    \cmidrule(r){2-5}\cmidrule{6-8}
             & \rheader{\bwb SItp+\zzz}
             & \rheader{SItp+\zzz}
             & \rheader{\bwb MS Itp}
             & \rheader{\bwb MS}
             & \rheader{MS Itp}
             & \rheader{MS}
             & \rheader{MS, \cvc, \zzz}                                                                                                \\

             \cmidrule(r){2-2}
             \cmidrule(r){3-3}
             \cmidrule(r){4-4}
             \cmidrule(r){5-5}
             \cmidrule(r){6-6}
             \cmidrule(r){7-7}
             \cmidrule{8-8}

    \OK      & 30 & 29 & 30 & 30 & 29        & 30        & 30         \\
    \NOK     & 18 & 18 & 18 & 18 & 18        & 18         & 18         \\
    \UNK     & 32 & 35 & 11 & 32 & -         & 6          & 5          \\
    \TOUT    & 16 & 30 & -  & 40 & 13        & 35         & 38         \\
    \OOM     & 4  & 4  & 1  & 2  & 2         & 1          & 1          \\
    \FAIL    & 8  & 5  & 58 & -  & 46        & 9          & 9          \\
    
    % \midrule
    %   & 14,510.35s & 14,457.25s & 5,016.94s & 16,470.74s & 8,246.31s & 15,806.49s & 15,689.53s \\
    \midrule
    \OK,\NOK & 51 & 70 & 48 & 70 & 83 & 93 &  91 \\
    \bottomrule
\end{tabular}



==> tab/tab_eval_reach_smt_svcomp.tex <==
\begin{tabular}{lr@{\hspace{1em}}r@{\hspace{1em}}r@{\hspace{1em}}r@{\hspace{1em}}r@{\hspace{1em}}r@{\hspace{1em}}c}
    \toprule
    & \multicolumn{4}{c}{Integer} & \multicolumn{3}{c}{Bitvector}                                                             \\
    \cmidrule(r){2-5}\cmidrule{6-8}
             & \rheader{\bwb SItp+\zzz}
             & \rheader{SItp+\zzz}
             & \rheader{\bwb MS Itp}
             & \rheader{\bwb MS}
             & \rheader{MS Itp}
             & \rheader{MS}
             & \rheader{MS, \cvc, \zzz}                                                                                                \\

             \cmidrule(r){2-2}
             \cmidrule(r){3-3}
             \cmidrule(r){4-4}
             \cmidrule(r){5-5}
             \cmidrule(r){6-6}
             \cmidrule(r){7-7}
             \cmidrule{8-8}

    \OK      & 15 & 17 & 16 & 14 & 17        & 12        & 12         \\
    \NOK     & 4 & 4 & 4 & 4 & 4        & 4         & 4         \\
    \UNK     & 32 & 35 & 11 & 32 & -         & 6          & 5          \\
    \TOUT    & 29 & 30 & 4  & 40 & 13        & 35         & 38         \\
    \OOM     & 4  & 4  & 1  & 2  & 2         & 1          & 1          \\
    \FAIL    & 8  & 5  & 58 & -  & 46        & 9          & 9          \\
    
    % \midrule
    %   & 14,510.35s & 14,457.25s & 5,016.94s & 16,470.74s & 8,246.31s & 15,806.49s & 15,689.53s \\
    \midrule
    \OK,\NOK & 71 & 70 & 21 & 70 & 83 & 93 &  91 \\
    \bottomrule
\end{tabular}


